Realtime-Capable Hybrid Spiking Neural Networks for Neural Decoding of Cortical Activity

Intra-cortical brain-machine interfaces (iBMIs) present a promising solution to restoring and decoding brain activity lost due to injury. However, patients with such neuroprosthetics suffer from permanent skull openings resulting from the devices' bulky wiring. This drives the development of wireless iBMIs, which demand low power consumption and small device footprint. Most recently, spiking neural networks (SNNs) have been researched as potential candidates for low-power neural decoding. In this work, we present the next step of utilizing SNNs for such tasks, building on the recently published results of the 2024 Grand Challenge on Neural Decoding Challenge for Motor Control of non-Human Primates. We optimize our model architecture to exceed the existing state of the art on the Primate Reaching dataset while maintaining similar resource demand through various compression techniques. We further focus on implementing a realtime-capable version of the model and discuss the implications of this architecture. With this, we advance one step towards latency-free decoding of cortical spike trains using neuromorphic technology, ultimately improving the lives of millions of paralyzed patients.

==> data/HPS/conv_channel.tex <==
224.71160924923328 0.45993584394454956
40.45233255692413 0.525789737701416
16.334562209764023 0.3566644489765167
60.60133481045998 0.42108044028282166
5.5614519189182285 0.497818261384964
13.113491237475102 0.43910419940948486
114.05070151605499 0.4532647132873535
66.94810439249176 0.4272300601005554
42.929565028899454 0.5435526371002197
47.9810037699251 0.4564681947231293
94.49729203551678 0.5117151737213135
153.19502683271932 0.5095414519309998
25.389101297354138 0.5008657574653625
88.38675969031831 0.4437015950679779
40.241914070443094 0.5061003565788269
81.9541466007737 0.5106759071350098
121.03025783849117 0.4052636921405792
44.681672116263925 0.4916248321533203
36.33694405304183 0.512349545955658
25.598438444642014 0.5618148446083069
27.071704671619965 0.4735218286514282
33.80513144632413 0.47308024764060974
20.972482091311225 0.44162803888320923
46.30747293892404 0.5118492245674133
67.21565968062642 0.32808351516723633
25.197857392665348 0.468524694442749
248.70408383849394 0.3120883107185364
59.64399101162076 0.34969279170036316
7.946618244258838 0.3678343892097473
36.180142263510255 0.47005006670951843
48.94519559425816 0.5652527809143066
51.87350209078591 0.48351895809173584
33.8665048108933 0.47355082631111145
66.76223721263757 0.3388618528842926
61.62324109464871 0.5287395119667053
109.15194116193815 0.39703986048698425
135.94308069315957 0.5105233192443848
54.638202948716355 0.46050432324409485
42.96046098876928 0.3801594078540802
4.638192536517504 0.3337802290916443
31.612945901020467 0.3451659381389618
166.54483286016224 0.4560140073299408
21.176915942472093 0.4753625690937042
87.20368773438756 0.44417262077331543
79.48317852577404 0.39846307039260864
42.623818249327556 0.4468592703342438
61.84685090428212 0.47519850730895996
34.326483572600424 0.412140429019928
26.95900938355977 0.5059142112731934
47.90824585022977 0.4550720155239105
71.9047085422198 0.5026651620864868
40.171689167205955 0.36095982789993286
43.334736948389285 0.3443441390991211
36.86521088006113 0.5368353128433228
42.41046857053299 0.5186737775802612
39.174775029347735 0.5269094109535217
44.10112584075524 0.5380277037620544
38.622127752150945 0.5186618566513062
39.827190747625316 0.6233993768692017
40.148245018844975 0.5903181433677673
38.76451453533642 0.576761782169342
40.76160354337418 0.6153431534767151
46.62142281576382 0.559240460395813

==> data/HPS/kernel_size.tex <==
0.9456102180141492 0.43317532539367676
16.19037423399229 0.45993584394454956
17.271032258857684 0.525789737701416
11.895842459768815 0.3566644489765167
6.68717934634179 0.42108044028282166
16.62451391703081 0.497818261384964
14.522158325977216 0.43910419940948486
14.565417924413916 0.4532647132873535
1.7771548864433455 0.4272300601005554
13.599617935797687 0.5435526371002197
7.453841359770188 0.4564681947231293
13.812894390207322 0.5117151737213135
7.0432158403080445 0.5095414519309998
17.36927658841817 0.5008657574653625
12.507178487215203 0.4437015950679779
15.830419505933982 0.5061003565788269
15.685744563099334 0.5106759071350098
14.412885268528719 0.4052636921405792
15.277597637256067 0.4916248321533203
15.592924979677264 0.512349545955658
16.56817054663409 0.5618148446083069
4.357944203241895 0.4735218286514282
16.177138094974243 0.47308024764060974
16.215989631084923 0.44162803888320923
13.589128591340849 0.5118492245674133
9.586281559541854 0.32808351516723633
12.99921938968061 0.468524694442749
11.349573121353151 0.3120883107185364
17.643984068506306 0.34969279170036316
10.671907891881226 0.3678343892097473
16.621482371441502 0.47005006670951843
14.467217568600347 0.5652527809143066
16.613786550358473 0.48351895809173584
12.184629223543448 0.47355082631111145
12.775864580957677 0.3388618528842926
4.629229338809268 0.5287395119667053
7.487764957864458 0.39703986048698425
8.374920016555032 0.5105233192443848
8.666251803803647 0.46050432324409485
11.636230817693349 0.3801594078540802
3.4696811336388915 0.3337802290916443
18.304491663784574 0.3451659381389618
7.751052713293736 0.4560140073299408
10.754523334369532 0.4753625690937042
11.041269145104515 0.44417262077331543
14.612151045724747 0.39846307039260864
16.502140537536306 0.4468592703342438
16.374634094438505 0.47519850730895996
16.294563703654863 0.412140429019928
13.582683952316572 0.5059142112731934
18.61705186866221 0.4550720155239105
17.278744897120387 0.5026651620864868
13.955168805789336 0.36095982789993286
16.476185801506624 0.3443441390991211
18.319026610199472 0.5368353128433228
16.949854224263454 0.5186737775802612
18.202953067541188 0.5269094109535217
18.339390388794815 0.5380277037620544
15.18870998911545 0.5186618566513062
19.894607095009547 0.6233993768692017
17.673585306527563 0.5903181433677673
16.27552235683884 0.576761782169342
26.60092883896744 0.6153431534767151
18.04469801170215 0.559240460395813

==> data/HPS/n_lif.tex <==
42.11048009005644 0.43317532539367676
98.84220153264053 0.45993584394454956
94.32392462066034 0.525789737701416
2.304136982430216 0.3566644489765167
88.7623903324336 0.42108044028282166
123.1558794115542 0.497818261384964
125.57671200285621 0.43910419940948486
99.80822473275862 0.4532647132873535
22.495008019194543 0.4272300601005554
76.44054386989869 0.5435526371002197
61.910202092687875 0.4564681947231293
86.52834159478356 0.5117151737213135
72.63243102500131 0.5095414519309998
67.65061347327911 0.5008657574653625
86.08607115170092 0.4437015950679779
92.08007324665789 0.5061003565788269
78.61677001742704 0.5106759071350098
110.69545031167007 0.4052636921405792
99.15357752313851 0.4916248321533203
56.65840606744964 0.512349545955658
55.63792227149776 0.5618148446083069
59.65533721968825 0.4735218286514282
69.77298621688908 0.47308024764060974
53.60907464264241 0.44162803888320923
46.36162212364501 0.5118492245674133
80.84356311934528 0.32808351516723633
51.30011659002355 0.468524694442749
61.82805075444833 0.3120883107185364
82.43820153695839 0.34969279170036316
44.639111998880416 0.3678343892097473
29.12182101716235 0.47005006670951843
43.55062145284524 0.5652527809143066
60.57863160816834 0.48351895809173584
40.542002588195 0.47355082631111145
9.070464657382576 0.3388618528842926
65.67739934555915 0.5287395119667053
94.53672091740003 0.39703986048698425
108.46985390661186 0.5105233192443848
69.43786820975895 0.46050432324409485
61.31627065984425 0.3801594078540802
77.380442907597 0.3337802290916443
49.456181223492585 0.3451659381389618
62.55554687815511 0.4560140073299408
54.59949494566577 0.4753625690937042
85.7864456428089 0.44417262077331543
32.76748497459622 0.39846307039260864
47.572349438640245 0.4468592703342438
46.85372417615813 0.47519850730895996
35.36850195136149 0.412140429019928
116.92314259092814 0.5059142112731934
61.463617982941884 0.4550720155239105
55.05005153295665 0.5026651620864868
68.58689794792545 0.36095982789993286
40.551082263295605 0.3443441390991211
53.52587841692549 0.5368353128433228
53.81894159267218 0.5186737775802612
60.659713480383864 0.5269094109535217
54.91396460771938 0.5380277037620544
54.07347977214987 0.5186618566513062
55.90562820779012 0.6233993768692017
51.03265434523889 0.5903181433677673
56.74265203666226 0.576761782169342
56.359843650604226 0.6153431534767151

==> data/HPS/n_lif_layer.tex <==
2 0.43317532539367676
1 0.45993584394454956
2 0.525789737701416
2 0.3566644489765167
2 0.42108044028282166
2 0.497818261384964
2 0.43910419940948486
2 0.4532647132873535
2 0.4272300601005554
2 0.5435526371002197
2 0.4564681947231293
2 0.5117151737213135
2 0.5095414519309998
1 0.5008657574653625
2 0.4437015950679779
2 0.5061003565788269
2 0.5106759071350098
2 0.4052636921405792
2 0.4916248321533203
2 0.512349545955658
2 0.5618148446083069
2 0.4735218286514282
2 0.47308024764060974
2 0.44162803888320923
2 0.5118492245674133
1 0.32808351516723633
1 0.468524694442749
2 0.3120883107185364
1 0.34969279170036316
2 0.3678343892097473
2 0.47005006670951843
2 0.5652527809143066
2 0.48351895809173584
2 0.47355082631111145
2 0.3388618528842926
2 0.5287395119667053
2 0.39703986048698425
2 0.5105233192443848
2 0.46050432324409485
2 0.3801594078540802
2 0.3337802290916443
2 0.3451659381389618
2 0.4560140073299408
2 0.4753625690937042
2 0.44417262077331543
2 0.39846307039260864
2 0.4468592703342438
2 0.47519850730895996
2 0.412140429019928
2 0.5059142112731934
2 0.4550720155239105
2 0.5026651620864868
2 0.36095982789993286
2 0.3443441390991211
2 0.5368353128433228
2 0.5186737775802612
2 0.5269094109535217
2 0.5380277037620544
2 0.5186618566513062
2 0.6233993768692017
2 0.5903181433677673
2 0.576761782169342
2 0.6153431534767151

==> data/HPS/seq_len.tex <==
753.6658759955021 0.43317532539367676
1496.931472735003 0.45993584394454956
1741.2503733537592 0.525789737701416
248.2597976663621 0.3566644489765167
950.0103187005872 0.42108044028282166
1632.9778703782192 0.497818261384964
1544.2153723646006 0.43910419940948486
1596.1267149187913 0.4532647132873535
1049.423446087994 0.4272300601005554
1923.5933266818195 0.5435526371002197
502.88281855695527 0.4564681947231293
1185.958148704547 0.5117151737213135
2106.8806657521104 0.5095414519309998
2252.4396527246417 0.5008657574653625
1088.053048517367 0.4437015950679779
1202.6682143984538 0.5061003565788269
1307.4037014807843 0.5106759071350098
1962.451278323245 0.4052636921405792
783.0191286696129 0.4916248321533203
2959.4979918692034 0.512349545955658
2520.442373132053 0.5618148446083069
389.89536135634705 0.4735218286514282
2786.3959235844904 0.47308024764060974
2965.931393226354 0.44162803888320923
2654.9486451753937 0.5118492245674133
1899.5035461603968 0.32808351516723633
1379.0364697060668 0.468524694442749
1780.3458740869353 0.3120883107185364
1392.1025424284185 0.34969279170036316
676.4394025461717 0.3678343892097473
2268.959741772524 0.47005006670951843
1743.5902176991433 0.5652527809143066
1745.8796090925982 0.48351895809173584
211.83141125462362 0.47355082631111145
1925.426182917575 0.3388618528842926
1642.726819538556 0.5287395119667053
939.3827452092016 0.39703986048698425
1258.0342290813721 0.5105233192443848
1638.0326532987795 0.46050432324409485
2267.396768045103 0.3801594078540802
2068.655287057615 0.3337802290916443
1704.4640456395236 0.3451659381389618
681.9538358797346 0.4560140073299408
1128.1212333590688 0.4753625690937042
1464.0102752551134 0.44417262077331543
1998.3054587719994 0.39846307039260864
2390.344046642965 0.4468592703342438
2354.6537667991292 0.47519850730895996
2129.377362023865 0.412140429019928
1819.131115943888 0.5059142112731934
2410.0873841537295 0.4550720155239105
498.94494809401743 0.5026651620864868
2155.95560382143 0.36095982789993286
1612.7667200477672 0.3443441390991211
2634.2921295819137 0.5368353128433228
3272.856515408156 0.5186737775802612
3238.2515306682526 0.5269094109535217
3262.066349441337 0.5380277037620544
3260.9342869994903 0.5186618566513062
3438.136783035816 0.6233993768692017
3861.2752284429994 0.5903181433677673
3840.7486760219385 0.576761782169342
3870.1732585833406 0.6153431534767151

==> data/traj_label.tex <==
-0.0034446716 0.0002403259
-0.0033721924 0.0001258850
-0.0033187866 0.0000152588
-0.0032730103 -0.0000915527
-0.0032272339 -0.0002059937
-0.0031661987 -0.0003166199
-0.0030822754 -0.0004158020
-0.0029830933 -0.0005073547
-0.0028686523 -0.0005874634
-0.0027465820 -0.0006523132
-0.0026245117 -0.0006904602
-0.0025100708 -0.0007057190
-0.0024070740 -0.0007095337
-0.0023231506 -0.0007133484
-0.0022659302 -0.0007133484
-0.0022239685 -0.0007057190
-0.0021896362 -0.0007057190
-0.0021476746 -0.0007095337
-0.0020637512 -0.0007019043
-0.0019264221 -0.0006980896
-0.0017318726 -0.0007057190
-0.0014648438 -0.0007324219
-0.0011177063 -0.0007934570
-0.0006752014 -0.0009002686
-0.0001144409 -0.0010719299
0.0005874634 -0.0013351440
0.0014686584 -0.0017051697
0.0025672913 -0.0021934509
0.0039024353 -0.0028266907
0.0054931641 -0.0036125183
0.0073738098 -0.0045585632
0.0095787048 -0.0056953430
0.0121650696 -0.0070610046
0.0152015686 -0.0086975098
0.0187416077 -0.0106468201
0.0228385925 -0.0129318237
0.0275230408 -0.0155754089
0.0328102112 -0.0185890198
0.0386886597 -0.0219650269
0.0450935364 -0.0256652832
0.0518379211 -0.0295829773
0.0585899353 -0.0335235596
0.0649299622 -0.0372467041
0.0704879761 -0.0405387878
0.0751037598 -0.0432968140
0.0787925720 -0.0455436707
0.0816688538 -0.0473747253
0.0839157104 -0.0489273071
0.0857658386 -0.0503768921
0.0874977112 -0.0519332886
0.0894126892 -0.0538215637
0.0917968750 -0.0562362671
0.0947532654 -0.0592651367
0.0980949402 -0.0628204346
0.1013450623 -0.0666198730
0.1039581299 -0.0703430176
0.1056938171 -0.0738296509
0.1066932678 -0.0771522522
0.1072921753 -0.0805130005
0.1078605652 -0.0841407776
0.1087341309 -0.0882568359
0.1101913452 -0.0930519104
0.1124992371 -0.0987205505
0.1158409119 -0.1054191589
0.1201934814 -0.1131324768
0.1251945496 -0.1215400696
0.1301002502 -0.1299819946
0.1340560913 -0.1376838684
0.1365203857 -0.1441993713
0.1374053955 -0.1495513916
0.1368865967 -0.1540260315
0.1352233887 -0.1580009460
0.1327095032 -0.1618995667
0.1296882629 -0.1661949158
0.1265563965 -0.1714019775
0.1237106323 -0.1780395508
0.1214752197 -0.1864852905
0.1199417114 -0.1967468262
0.1188011169 -0.2082290649
0.1173934937 -0.2196998596
0.1149978638 -0.2298164368
0.1112670898 -0.2378578186
0.1063575745 -0.2439231873
0.1006698608 -0.2485580444
0.0945968628 -0.2523880005
0.0884895325 -0.2560920715
0.0826644897 -0.2604007721
0.0774002075 -0.2660484314
0.0728912354 -0.2736568451
0.0691909790 -0.2834510803
0.0661506653 -0.2948875427
0.0633811951 -0.3065338135
0.0603981018 -0.3165531158
0.0568542480 -0.3236598969
0.0526428223 -0.3277034760
0.0478248596 -0.3293590546
0.0425109863 -0.3295383453
0.0367774963 -0.3291606903
0.0307159424 -0.3292198181
0.0244178772 -0.3307991028
0.0179557800 -0.3349418640
0.0113945007 -0.3423538208
0.0047569275 -0.3529834747
-0.0019607544 -0.3656406403
-0.0087814331 -0.3780174255
-0.0157165527 -0.3876152039
-0.0227584839 -0.3931083679
-0.0299034119 -0.3947734833
-0.0371932983 -0.3937625885
-0.0446968079 -0.3913745880
-0.0525131226 -0.3888874054
-0.0607757568 -0.3875656128
-0.0696029663 -0.3886165619
-0.0790939331 -0.3929843903
-0.0892105103 -0.4008865356
-0.0996704102 -0.4113349915
-0.1099395752 -0.4220905304
-0.1193695068 -0.4305019379
-0.1275329590 -0.4348888397
-0.1343727112 -0.4351902008
-0.1400871277 -0.4324111938
-0.1450004578 -0.4278411865
-0.1494789124 -0.4227752686
-0.1539459229 -0.4185047150
-0.1588668823 -0.4163475037
-0.1647109985 -0.4175567627
-0.1718063354 -0.4229412079
-0.1800804138 -0.4323215485
-0.1888885498 -0.4440841675
-0.1970214844 -0.4552516937
-0.2031631470 -0.4626235962
-0.2066192627 -0.4644622803
-0.2075653076 -0.4610424042
-0.2066459656 -0.4537582397
-0.2045974731 -0.4441947937
-0.2021522522 -0.4339103699
-0.2000427246 -0.4245109558
-0.1990089417 -0.4176292419
-0.1996879578 -0.4146900177
-0.2023849487 -0.4164428711
-0.2068405151 -0.4224452972
-0.2120704651 -0.4307727814
-0.2164535522 -0.4382057190
-0.2183189392 -0.4414253235
-0.2168045044 -0.4387378693
-0.2121009827 -0.4305572510
-0.2049446106 -0.4183864594
-0.1961822510 -0.4038639069
-0.1866264343 -0.3885364532
-0.1770668030 -0.3738727570
-0.1682281494 -0.3612213135
-0.1606559753 -0.3515434265
-0.1545295715 -0.3449974060
-0.1494789124 -0.3406009674
-0.1446647644 -0.3362751007
-0.1391525269 -0.3297176361
-0.1324348450 -0.3196449280
-0.1246299744 -0.3061771393
-0.1161804199 -0.2901935577
-0.1075401306 -0.2726726532
-0.0991058350 -0.2545375824
-0.0912361145 -0.2366638184
-0.0842170715 -0.2198581696
-0.0782203674 -0.2047557831
-0.0732498169 -0.1915931702
-0.0690765381 -0.1800136566
-0.0652313232 -0.1690864563
-0.0611915588 -0.1577434540
-0.0566635132 -0.1453952789
-0.0516090393 -0.1321334839
-0.0461502075 -0.1183986664
-0.0404624939 -0.1046352386
-0.0346946716 -0.0912322998
-0.0289726257 -0.0785274506
-0.0234336853 -0.0668048859
-0.0181961060 -0.0562953949
-0.0133323669 -0.0471267700
-0.0088882446 -0.0392799377
-0.0048484802 -0.0325794220
-0.0011901855 -0.0267257690
0.0020980835 -0.0214328766
0.0049858093 -0.0165634155
0.0073966980 -0.0121402740
0.0092735291 -0.0082359314
0.0106010437 -0.0048866272
0.0114021301 -0.0020961761
0.0117073059 0.0001487732
0.0115814209 0.0018844604
0.0111083984 0.0031700134
0.0103797913 0.0040798187
0.0094604492 0.0046825409
0.0083923340 0.0050334930
0.0071907043 0.0051708221
0.0058746338 0.0051212311
0.0045051575 0.0049228668
0.0031776428 0.0046176910
0.0019912720 0.0042457581
0.0010147095 0.0038414001
0.0002899170 0.0034313202
-0.0001792908 0.0030345917
-0.0004119873 0.0026645660
-0.0004425049 0.0023384094
-0.0003242493 0.0020618439
-0.0001106262 0.0018348694
0.0001564026 0.0016517639
0.0004310608 0.0015029907
0.0006752014 0.0013847351
0.0008697510 0.0012912750
0.0010032654 0.0012302399
0.0010833740 0.0011978149
0.0011291504 0.0011882782
0.0011634827 0.0012016296
0.0012016296 0.0012340546
0.0012474060 0.0012760162
0.0013122559 0.0013198853
0.0013961792 0.0013599396
0.0014877319 0.0013790131
0.0015716553 0.0013637543
0.0016403198 0.0013160706
0.0016899109 0.0012454987
0.0017166138 0.0011653900
0.0017280579 0.0010967255
0.0017280579 0.0010490417
0.0017204285 0.0010299683
0.0017204285 0.0010471344
0.0017318726 0.0011005402
0.0017585754 0.0011863708
0.0018119812 0.0013027191
0.0018844604 0.0014419556
0.0019645691 0.0015907288
0.0020484924 0.0017375946
0.0021209717 0.0018730164
0.0021743774 0.0019950867
0.0022125244 0.0021076202
0.0022239685 0.0022182465
0.0022087097 0.0023269653
0.0021705627 0.0024375916
0.0021018982 0.0025577545
0.0020179749 0.0026874542
0.0019187927 0.0028228760
0.0018005371 0.0029582977
0.0016670227 0.0030746460
0.0015106201 0.0031509399
0.0013389587 0.0031814575
0.0011672974 0.0031700134
0.0010223389 0.0031242371
0.0009155273 0.0030612946
0.0008544922 0.0029983521
0.0008506775 0.0029487610
0.0008964539 0.0029239655
0.0009918213 0.0029315948
0.0011291504 0.0029830933
0.0012855530 0.0030765533
0.0014495850 0.0031948090
0.0016059875 0.0033168793
0.0017242432 0.0034179688
0.0018005371 0.0034790039
0.0018386841 0.0034885406
0.0018424988 0.0034484863
0.0018348694 0.0033645630
0.0018196106 0.0032444000
0.0018005371 0.0031013489
0.0017890930 0.0029487610
0.0017967224 0.0028038025
0.0018196106 0.0026760101
0.0018463135 0.0025691986
0.0018653870 0.0024719238
0.0018653870 0.0023784637
0.0018463135 0.0022869110
0.0018043518 0.0022010803
0.0017471313 0.0021324158
0.0016860962 0.0020847321
0.0016174316 0.0020675659
0.0015373230 0.0020847321
0.0014495850 0.0021419525
0.0013504028 0.0022430420
0.0012359619 0.0023937225
0.0010986328 0.0025939941
0.0009384155 0.0028285980
0.0007400513 0.0030765533
0.0004997253 0.0033168793
0.0002212524 0.0035362244
-0.0000801086 0.0037269592
-0.0003776550 0.0038890839
-0.0006599426 0.0040302277
-0.0009155273 0.0041618347
-0.0011291504 0.0042915344
-0.0013008118 0.0044269562
-0.0014343262 0.0045814514
-0.0015258789 0.0047626495
-0.0015792847 0.0049571991
-0.0015945435 0.0051441193
-0.0015640259 0.0052947998
-0.0014839172 0.0053787231
-0.0013656616 0.0053844452
-0.0012168884 0.0053234100
-0.0010604858 0.0052185059
-0.0009117126 0.0050868988
-0.0007858276 0.0049533844
-0.0006980896 0.0048389435
-0.0006446838 0.0047607422
-0.0006332397 0.0047378540
-0.0006599426 0.0047721863
-0.0007133484 0.0048484802
-0.0007858276 0.0049362183
-0.0008697510 0.0049991608
-0.0009498596 0.0050125122
-0.0010070801 0.0049667358
-0.0010414124 0.0048599243
-0.0010452271 0.0047035217
-0.0010147095 0.0045089722
-0.0009498596 0.0042896271
-0.0008506775 0.0040645599
-0.0007324219 0.0038528442
-0.0005989075 0.0036697388
-0.0004463196 0.0035228729
-0.0002861023 0.0034046173
-0.0001220703 0.0032978058
0.0000419617 0.0031909943
0.0001983643 0.0030765533
0.0003433228 0.0029582977
0.0004615784 0.0028400421
0.0005607605 0.0027256012
0.0006370544 0.0026226044
0.0006980896 0.0025367737
0.0007591248 0.0024719238
0.0008201599 0.0024375916
0.0008926392 0.0024356842
0.0009841919 0.0024623871
0.0011024475 0.0025081635
0.0012397766 0.0025596619
0.0013923645 0.0026092529
0.0015640259 0.0026493073
0.0017585754 0.0026855469
0.0019645691 0.0027198792
0.0021896362 0.0027523041
0.0024414062 0.0027904510
0.0027236938 0.0028400421
0.0030479431 0.0029106140
0.0034255981 0.0030097961
0.0038528442 0.0031394958
0.0043106079 0.0032863617
0.0047836304 0.0034294128
0.0052452087 0.0035572052
0.0056838989 0.0036602020
0.0061073303 0.0037403107
0.0065345764 0.0038070679
0.0069808960 0.0038700104
0.0074653625 0.0039424896
0.0080184937 0.0040435791
0.0086822510 0.0041923523
0.0094871521 0.0044097900
0.0104331970 0.0047035217
0.0115127563 0.0050640106
0.0126686096 0.0054702759
0.0138015747 0.0058803558
0.0148200989 0.0062522888
0.0156822205 0.0065650940
0.0164337158 0.0068244934
0.0171394348 0.0070476532
0.0178718567 0.0072612762
0.0187149048 0.0074882507
0.0197334290 0.0077495575
0.0209960938 0.0080623627
0.0225219727 0.0084247589
0.0242614746 0.0088157654
0.0261077881 0.0091819763
0.0279350281 0.0094699860
0.0296821594 0.0096530914
0.0313873291 0.0097351074
0.0331497192 0.0097484589
0.0350685120 0.0097274780
0.0372428894 0.0097064972
0.0397644043 0.0097179413
0.0427284241 0.0097980499
0.0462646484 0.0099868774
0.0504760742 0.0103244781
0.0553474426 0.0108261108
0.0607185364 0.0114765167
0.0662651062 0.0122299194
0.0716018677 0.0130157471
0.0765304565 0.0137939453
0.0811195374 0.0145549774
0.0855827332 0.0152988434
0.0901908875 0.0160388947
0.0952262878 0.0168018341
0.1009902954 0.0176181793
0.1078224182 0.0185356140
0.1160430908 0.0196208954
0.1258239746 0.0209217072
0.1370391846 0.0224399567
0.1491050720 0.0241088867
0.1609916687 0.0257854462
0.1716194153 0.0273208618
0.1803932190 0.0286636353
0.1874084473 0.0298728943
0.1931648254 0.0310649872
0.1982574463 0.0323600769
0.2033195496 0.0338745117
0.2090225220 0.0357112885
0.2160644531 0.0379543304
0.2249908447 0.0406551361
0.2358970642 0.0437736511
0.2481651306 0.0471324921
0.2604255676 0.0504169464
0.2711677551 0.0532894135
0.2796173096 0.0555515289
0.2860336304 0.0572166443
0.2912406921 0.0584316254
0.2962074280 0.0593910217
0.3019866943 0.0603275299
0.3096885681 0.0614986420
0.3204917908 0.0631828308
0.3354682922 0.0656375885
0.3552131653 0.0690212250
0.3793601990 0.0733070374
0.4063072205 0.0782203674
0.4335060120 0.0833053589
0.4585685730 0.0881290436
0.4805488586 0.0925006866
0.5000610352 0.0965042114
0.5184745789 0.1003322601
0.5372657776 0.1041755676
0.5578804016 0.1082191467
0.5817909241 0.1126651764
0.6103820801 0.1177463531
0.6445274353 0.1236495972
0.6838378906 0.1303424835
0.7258224487 0.1374034882
0.7658538818 0.1440200806
0.7990036011 0.1493110657
0.8227386475 0.1528644562
0.8377876282 0.1548805237
0.8466529846 0.1558628082
0.8521537781 0.1563510895
0.8571205139 0.1568603516
0.8644599915 0.1579074860
0.8771781921 0.1600246429
0.8979911804 0.1636962891
0.9282951355 0.1691684723
0.9669723511 0.1762218475
1.0097351074 0.1840534210
1.0498847961 0.1914215088
1.0811538696 0.1971435547
1.1009063721 0.2006721497
1.1105651855 0.2021770477
1.1135559082 0.2021923065
1.1137046814 0.2013301849
1.1149215698 0.2002315521
1.1212348938 0.1995697021
1.1364250183 0.1999721527
1.1630592346 0.2018527985
1.2010726929 0.2051677704
1.2465438843 0.2092113495
1.2917976379 0.2126369476
1.3284645081 0.2139987946
1.3520126343 0.2125473022
1.3628730774 0.2084140778
1.3638534546 0.2021389008
1.3582572937 0.1942996979
1.3499832153 0.1855030060
1.3436126709 0.1764068604
1.3439426422 0.1676826477
1.3551483154 0.1599082947
1.3793201447 0.1533813477
1.4147548676 0.1479358673
1.4551525116 0.1428890228
1.4911499023 0.1372432709
1.5145187378 0.1301193237
1.5221614838 0.1211738586
1.5162391663 0.1105861664
1.5014247894 0.0987625122
1.4828929901 0.0861148834
1.4659290314 0.0730018616
1.4560146332 0.0597419739
1.4586181641 0.0465965271
1.4782123566 0.0337581635
1.5164394379 0.0213241577
1.5702972412 0.0093059540
1.6313762665 -0.0023460388
1.6872844696 -0.0136966705
1.7264442444 -0.0247764587
1.7436294556 -0.0355911255
1.7407264709 -0.0461292267
1.7229652405 -0.0563926697
1.6958055496 -0.0664043427
1.6642837524 -0.0762119293
1.6333112717 -0.0859069824
1.6074991226 -0.0955867767
1.5896883011 -0.1052551270
1.5787429810 -0.1146812439
1.5687851906 -0.1233215332
1.5519981384 -0.1305141449
1.5233988762 -0.1358451843
1.4827227592 -0.1393013000
1.4325537682 -0.1411342621
1.3766236305 -0.1417198181
1.3196377754 -0.1415576935
1.2669215202 -0.1412467957
1.2236602306 -0.1414146423
1.1944497824 -0.1426753998
1.1826974154 -0.1455326080
1.1893368959 -0.1502056122
1.2115007639 -0.1564559937
1.2418363094 -0.1634674072
1.2692521811 -0.1699352264
1.2827808857 -0.1745777130
1.2770172358 -0.1768283844
1.2535712719 -0.1770324707
1.2177336216 -0.1760025024
1.1753127575 -0.1745948792
1.1318023205 -0.1735973358
1.0923538208 -0.1737365723
1.0613374710 -0.1756076813
1.0412769318 -0.1794967651
1.0316610336 -0.1851787567
1.0283646584 -0.1917819977
1.0244774818 -0.1979370117
1.0132818222 -0.2022895813
0.9917221069 -0.2041339874
0.9609737396 -0.2035617828
0.9242553711 -0.2010784149
0.8849945068 -0.1972789764
0.8463068008 -0.1927566528
0.8109674454 -0.1880893707
0.7814197540 -0.1838245392
0.7593708038 -0.1803779602
0.7448959351 -0.1777935028
0.7356348038 -0.1755390167
0.7269353867 -0.1725425720
0.7137689590 -0.1676425934
0.6934537888 -0.1602516174
0.6664333344 -0.1505470276
0.6347579956 -0.1390991211
0.6006698608 -0.1265258789
0.5662727356 -0.1134128571
0.5335798264 -0.1003074646
0.5044670105 -0.0877113342
0.4804306030 -0.0760383606
0.4620761871 -0.0655269623
0.4485893250 -0.0561790466
0.4376888275 -0.0477924347
0.4264869690 -0.0400753021
0.4129924774 -0.0328140259
0.3968944550 -0.0259647369
0.3790454865 -0.0195751190
0.3606262207 -0.0136985779
0.3427639008 -0.0083541870
0.3265171051 -0.0035247803
0.3129100800 0.0008296967
0.3028354645 0.0047760010
0.2968139648 0.0083904266
0.2946491241 0.0117454529
0.2951412201 0.0148849487
0.2961883545 0.0178050995
0.2955684662 0.0204811096
0.2920665741 0.0228977203
0.2858333588 0.0250587463
0.2777366638 0.0269908905
0.2687511444 0.0287265778
0.2598056793 0.0303058624
0.2517871857 0.0317935944
0.2455368042 0.0332832336
0.2417278290 0.0348663330
0.2406044006 0.0365905762
0.2416992188 0.0384197235
0.2437496185 0.0401897430
0.2450256348 0.0416679382
0.2440795898 0.0426845551
0.2403984070 0.0432243347
0.2343368530 0.0434303284
0.2265834808 0.0434894562
0.2177848816 0.0435619354
0.2084827423 0.0437774658
0.1992321014 0.0442466736
0.1906318665 0.0450878143
0.1831359863 0.0463733673
0.1767616272 0.0480728149
0.1709041595 0.0500030518
0.1644058228 0.0518264771
0.1560173035 0.0531921387
0.1450366974 0.0539379120
0.1315021515 0.0541572571
0.1158390045 0.0540771484
0.0985183716 0.0539588928
0.0799751282 0.0540771484
0.0606193542 0.0547180176
0.0408401489 0.0561809540
0.0209827423 0.0587387085
0.0013046265 0.0625820160
-0.0180187225 0.0677299500
-0.0368156433 0.0739707947
-0.0548362732 0.0808334351
-0.0717010498 0.0876064301
-0.0869789124 0.0935840607
-0.1003723145 0.0983943939
-0.1118144989 0.1020889282
-0.1214447021 0.1049671173
-0.1295490265 0.1073875427
-0.1365356445 0.1097202301
-0.1428966522 0.1123256683
-0.1490459442 0.1154479980
-0.1550960541 0.1190738678
-0.1606712341 0.1227931976
-0.1648979187 0.1258163452
-0.1668167114 0.1272926331
-0.1659832001 0.1267662048
-0.1626510620 0.1243438721
-0.1574497223 0.1204357147
-0.1510372162 0.1154975891
-0.1440143585 0.1099624634
-0.1369361877 0.1042423248
-0.1303100586 0.0987262726
-0.1245460510 0.0937385559
-0.1198501587 0.0894451141
-0.1160793304 0.0857582092
-0.1127243042 0.0823268890
-0.1091556549 0.0786991119
-0.1049671173 0.0746021271
-0.1001319885 0.0700550079
-0.0948295593 0.0652256012
-0.0892620087 0.0602951050
-0.0836143494 0.0554237366
-0.0780735016 0.0507583618
-0.0728454590 0.0464439392
-0.0681343079 0.0426082611
-0.0640830994 0.0393276215
-0.0606880188 0.0365772247
-0.0577392578 0.0342006683
-0.0548400879 0.0319328308
-0.0515804291 0.0295009613
-0.0477676392 0.0267677307
-0.0434856415 0.0237655640
-0.0389461517 0.0206108093
-0.0343608856 0.0174293518
-0.0299110413 0.0143299103
-0.0257472992 0.0114040375
-0.0219974518 0.0087261200
-0.0187587738 0.0063552856
-0.0160865784 0.0043296814
-0.0139770508 0.0026626587
-0.0123634338 0.0013465881
-0.0111541748 0.0003662109
-0.0102691650 -0.0003051758
-0.0096683502 -0.0006904602
-0.0093307495 -0.0008163452
-0.0092411041 -0.0007209778
-0.0093917847 -0.0004310608
-0.0097656250 0.0000152588
-0.0103492737 0.0005836487
-0.0111293793 0.0012435913
-0.0120811462 0.0019626617
-0.0131607056 0.0027084351
-0.0142879486 0.0034389496
-0.0153446198 0.0041103363
-0.0162029266 0.0046730042
-0.0167961121 0.0051040649
-0.0171318054 0.0054111481
-0.0172576904 0.0056114197
-0.0172386169 0.0057296753
-0.0171337128 0.0058002472
-0.0170059204 0.0058536530
-0.0169258118 0.0059185028
-0.0169506073 0.0060234070
-0.0171070099 0.0061874390
-0.0173683167 0.0064086914
-0.0176563263 0.0066642761
-0.0178794861 0.0069293976
-0.0179843903 0.0071868896
-0.0179824829 0.0074405670
-0.0179080963 0.0077018738
-0.0178050995 0.0079822540
-0.0177192688 0.0082931519
-0.0176963806 0.0086421967
-0.0177783966 0.0090427399
-0.0180072784 0.0095062256
-0.0184116364 0.0100345612
-0.0189762115 0.0106201172
-0.0196323395 0.0112152100
-0.0202522278 0.0117416382
-0.0207004547 0.0121231079
-0.0209102631 0.0123195648
-0.0209045410 0.0123538971
-0.0207538605 0.0122699738
-0.0205364227 0.0121192932
-0.0203247070 0.0119533539
-0.0201873779 0.0118160248
-0.0201969147 0.0117530823
-0.0204105377 0.0118007660
-0.0208530426 0.0119800568
-0.0214843750 0.0122756958
-0.0221920013 0.0126304626
-0.0228595734 0.0129776001
-0.0234127045 0.0132846832
-0.0238494873 0.0135574341
-0.0242137909 0.0138168335
-0.0245437622 0.0140914917
-0.0248775482 0.0144042969
-0.0252609253 0.0147705078
-0.0257377625 0.0152149200
-0.0263557434 0.0157642365
-0.0271492004 0.0164241791
-0.0280914307 0.0171699524
-0.0290679932 0.0179290771
-0.0298786163 0.0185699463
-0.0303096771 0.0189514160
-0.0302524567 0.0190029144
-0.0297355652 0.0187416077
-0.0288562775 0.0182304382
-0.0277156830 0.0175323486
-0.0264148712 0.0167102814
-0.0250511169 0.0158367157
-0.0237274170 0.0149822235
-0.0225372314 0.0142097473
-0.0215358734 0.0135593414
-0.0207290649 0.0130405426
-0.0200481415 0.0126190186
-0.0193843842 0.0122261047
-0.0186500549 0.0118122101
-0.0178203583 0.0113601685
-0.0169448853 0.0108928680
-0.0160903931 0.0104446411
-0.0153102875 0.0100402832
-0.0146579742 0.0097064972
-0.0141792297 0.0094642639
-0.0139083862 0.0093345642
-0.0138607025 0.0093326569
-0.0140266418 0.0094528198
-0.0143413544 0.0096549988
-0.0146980286 0.0098762512
-0.0149860382 0.0100460052
-0.0151405334 0.0101242065
-0.0151634216 0.0101146698
-0.0150890350 0.0100421906
-0.0149631500 0.0099353790
-0.0148315430 0.0098247528
-0.0147418976 0.0097427368
-0.0147476196 0.0097198486
-0.0148944855 0.0097866058
-0.0152053833 0.0099582672
-0.0156669617 0.0102214813
-0.0162048340 0.0105247498
-0.0167007446 0.0107879639
-0.0170230865 0.0109252930
-0.0170993805 0.0108890533
-0.0169391632 0.0106906891
-0.0165977478 0.0103759766
-0.0161571503 0.0099983215
-0.0156860352 0.0096130371
-0.0152549744 0.0092678070
-0.0149307251 0.0090045929
-0.0147571564 0.0088558197
-0.0147514343 0.0088253021
-0.0148735046 0.0088882446
-0.0150394440 0.0089912415
-0.0151519775 0.0090770721
-0.0151634216 0.0091075897
-0.0150794983 0.0090827942
-0.0149345398 0.0090255737
-0.0147762299 0.0089530945
-0.0146331787 0.0088863373
-0.0145397186 0.0088443756
-0.0145320892 0.0088462830
-0.0146350861 0.0089073181
-0.0148487091 0.0090312958
-0.0151329041 0.0091934204
-0.0154037476 0.0093421936
-0.0155467987 0.0094146729
-0.0154838562 0.0093593597
-0.0152015686 0.0091686249
-0.0147342682 0.0088615417
-0.0141448975 0.0084743500
-0.0134925842 0.0080432892
-0.0128383636 0.0075988770
-0.0122413635 0.0071792603
-0.0117473602 0.0068149567
-0.0113906860 0.0065212250
-0.0111732483 0.0063056946
-0.0110626221 0.0061492920
-0.0109863281 0.0060100555
-0.0108642578 0.0058536530
-0.0106620789 0.0056610107
-0.0103855133 0.0054340363
-0.0100650787 0.0051994324
-0.0097465515 0.0049839020
-0.0094718933 0.0048084259
-0.0092830658 0.0046939850
-0.0092239380 0.0046634674
-0.0093364716 0.0047359467
-0.0096435547 0.0049152374
-0.0101375580 0.0051975250
-0.0107822418 0.0055599213
-0.0114994049 0.0059566498
-0.0121936798 0.0063419342
-0.0128021240 0.0066833496
-0.0133132935 0.0069732666
-0.0137577057 0.0072326660
-0.0141887665 0.0074939728
-0.0146617889 0.0077896118
-0.0152263641 0.0081481934
-0.0159339905 0.0085945129
-0.0168209076 0.0091457367
-0.0178871155 0.0098018646
-0.0190849304 0.0105285645
-0.0203075409 0.0112628937
-0.0214252472 0.0119361877
-0.0223655701 0.0125007629
-0.0231285095 0.0129489899
-0.0237503052 0.0132999420
-0.0242786407 0.0135746002
-0.0247726440 0.0138053894
-0.0253105164 0.0140323639
-0.0259761810 0.0143032074
-0.0268402100 0.0146617889
-0.0279254913 0.0151195526
-0.0291748047 0.0156497955
-0.0304374695 0.0161781311
-0.0315322876 0.0166091919
-0.0323276520 0.0168743134
-0.0328025818 0.0169658661
-0.0330352783 0.0169296265
-0.0331344604 0.0168266296
-0.0332088470 0.0167160034
-0.0333728790 0.0166568756
-0.0337352753 0.0167064667
-0.0343856812 0.0169105530
-0.0353775024 0.0172958374
-0.0366954803 0.0178508759
-0.0382099152 0.0185070038
-0.0396766663 0.0191459656
-0.0408344269 0.0196304321
-0.0415344238 0.0198783875
-0.0417881012 0.0198841095
-0.0416946411 0.0196781158
-0.0413684845 0.0193042755
-0.0409278870 0.0188121796
-0.0405101776 0.0182628632
-0.0402526855 0.0177268982
-0.0402774811 0.0172653198
-0.0406589508 0.0169258118
-0.0413532257 0.0167083740
-0.0421791077 0.0165500641
-0.0428714752 0.0163612366
-0.0432071686 0.0160732269
-0.0431365967 0.0156784058
-0.0427589417 0.0152378082
-0.0422401428 0.0148353577
-0.0417461395 0.0145339966
-0.0414142609 0.0143947601
-0.0413818359 0.0144634247
-0.0417709351 0.0147724152
-0.0426559448 0.0153388977
-0.0440254211 0.0161399841
-0.0457286835 0.0171070099
-0.0474758148 0.0181121826
-0.0489444733 0.0190200806
-0.0499401093 0.0197467804
-0.0504550934 0.0202713013
-0.0505847931 0.0206089020
-0.0504322052 0.0207881927
-0.0501003265 0.0208415985
-0.0497093201 0.0208091736
-0.0493907928 0.0207424164
-0.0492610931 0.0206832886
-0.0493602753 0.0206527710
-0.0495872498 0.0206127167
-0.0496845245 0.0204563141
-0.0493316650 0.0200538635
-0.0483169556 0.0193290710
-0.0466575623 0.0183067322
-0.0445442200 0.0170822144
-0.0422153473 0.0157737732
-0.0399074554 0.0144958496
-0.0378379822 0.0133438110
-0.0362167358 0.0124073029
-0.0352401733 0.0117702484
-0.0350551605 0.0114974976
-0.0357227325 0.0116214752
-0.0371952057 0.0121421814
-0.0393104553 0.0130214691
-0.0418910980 0.0142192841
-0.0448894501 0.0157470703
-0.0484199524 0.0176715851
-0.0526828766 0.0200881958
-0.0578765869 0.0230884552
-0.0641880035 0.0267505646
-0.0717945099 0.0311489105
-0.0808544159 0.0363445282
-0.0914630890 0.0423641205
-0.1035556793 0.0491657257
-0.1167850494 0.0565662384
-0.1304721832 0.0642261505
-0.1437835693 0.0717334747
-0.1560993195 0.0787715912
-0.1672430038 0.0852375031
-0.1773738861 0.0911865234
-0.1867990494 0.0967521667
-0.1959199905 0.1021251678
-0.2052373886 0.1075458527
-0.2153482437 0.1133136749
-0.2268905640 0.1197528839
-0.2403421402 0.1271133423
-0.2556953430 0.1353950500
-0.2721643448 0.1441822052
-0.2881803513 0.1526489258
-0.3020429611 0.1599082947
-0.3129291534 0.1655445099
-0.3212127686 0.1697883606
-0.3279285431 0.1732311249
-0.3342523575 0.1765289307
-0.3413839340 0.1803436279
-0.3505439758 0.1853466034
-0.3628883362 0.1921691895
-0.3792848587 0.2012825012
-0.3999109268 0.2127838135
-0.4238119125 0.2261734009
-0.4487552643 0.2402687073
-0.4718036652 0.2535037994
-0.4906282425 0.2646331787
-0.5045690536 0.2732982635
-0.5144786835 0.2799530029
-0.5218744278 0.2854042053
-0.5284099579 0.2905406952
-0.5358028412 0.2962989807
-0.5458498001 0.3036632538
-0.5602970123 0.3135967255
-0.5804128647 0.3267974854
-0.6062602997 0.3432884216
-0.6360015869 0.3620204926
-0.6659078598 0.3808631897
-0.6918659210 0.3974552155
-0.7116918564 0.4104900360
-0.7258605957 0.4201526642
-0.7362608910 0.4274425507
-0.7449922562 0.4335155487
-0.7540941238 0.4395446777
-0.7656569481 0.4467487335
-0.7818460464 0.4564056396
-0.8045248985 0.4696063995
-0.8343119621 0.4867000580
-0.8694834709 0.5066719055
-0.9056143761 0.5269336700
-0.9369750023 0.5441341400
-0.9593496323 0.5558185577
-0.9718360901 0.5614719391
-0.9761686325 0.5621051788
-0.9751042128 0.5593280792
-0.9715652466 0.5548439026
-0.9685066342 0.5503597260
-0.9689574242 0.5476131439
-0.9758542180 0.5482845306
-0.9913126230 0.5535907745
-1.0153824091 0.5635795593
-1.0449112654 0.5765132904
-1.0736063719 0.5889244080
-1.0945260525 0.5969886780
-1.1037969589 0.5985794067
-1.1018202305 0.5939407349
-1.0913701057 0.5846290588
-1.0757427216 0.5724716187
-1.0583806038 0.5593490601
-1.0429964066 0.5472640991
-1.0334343910 0.5382537842
-1.0329861641 0.5340499878
-1.0431323051 0.5354347229
-1.0622482300 0.5415611267
-1.0852313042 0.5498161316
-1.1051025391 0.5566253662
-1.1163349152 0.5591468811
-1.1172685623 0.5565147400
-1.1096458435 0.5495719910
-1.0967855453 0.5399513245
-1.0824546814 0.5294952393
-1.0704765320 0.5200500488
-1.0644226074 0.5133171082
-1.0672245026 0.5106735229
-1.0806503296 0.5129356384
-1.1043186188 0.5198936462
-1.1344861984 0.5297393799
-1.1640253067 0.5390777588
-1.1852216721 0.5442161560
-1.1940288544 0.5431518555
-1.1913356781 0.5361671448
-1.1805267334 0.5246963501
-1.1651172638 0.5102691650
-1.1482830048 0.4942779541
-1.1333255768 0.4781646729
-1.1238975525 0.4635353088
-1.1233730316 0.4519004822
-1.1334209442 0.4440650940
-1.1525268555 0.4395561218
-1.1753501892 0.4364166260
-1.1938629150 0.4316825867
-1.2007694244 0.4227180481
-1.1930675507 0.4085502625
-1.1723175049 0.3899345398
-1.1421890259 0.3683891296
-1.1065521240 0.3454208374
-1.0690727234 0.3223648071
-1.0333576202 0.3004379272
-1.0029354095 0.2807350159
-0.9805660248 0.2640647888
-0.9668998718 0.2506065369
-0.9593734741 0.2396774292
-0.9523372650 0.2297897339
-0.9393920898 0.2192382812
-0.9168758392 0.2069931030
-0.8851737976 0.1929893494
-0.8471412659 0.1777572632
-0.8062019348 0.1619796753
-0.7655525208 0.1462745667
-0.7280483246 0.1311912537
-0.6962356567 0.1172027588
-0.6721496582 0.1046791077
-0.6567039490 0.0938110352
-0.6489486694 0.0844955444
-0.6456375122 0.0763168335
-0.6417274475 0.0686340332
-0.6323509216 0.0608406067
-0.6152801514 0.0527153015
-0.5914154053 0.0444335938
-0.5631637573 0.0363082886
-0.5330543518 0.0286293030
-0.5033950806 0.0215797424


==> data/traj_pred.tex <==
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
0.0022157687 -0.0011790354
0.0055089833 -0.0034356872
0.0088021979 -0.0056923389
0.0120954125 -0.0079489907
0.0153886271 -0.0102056424
0.0186818417 -0.0124622942
0.0219750563 -0.0147189459
0.0252682709 -0.0169755977
0.0219750563 -0.0147189459
0.0186818417 -0.0124622942
0.0153886271 -0.0102056424
0.0120954125 -0.0079489907
0.0088021979 -0.0056923389
0.0055089833 -0.0034356872
0.0022157687 -0.0011790354
-0.0010774458 0.0010776163
-0.0027031940 -0.0023561191
-0.0043289422 -0.0057898545
-0.0059546903 -0.0092235899
-0.0075804385 -0.0126573253
-0.0092061866 -0.0160910607
-0.0108319348 -0.0195247961
-0.0124576829 -0.0229585315
-0.0140834311 -0.0263922669
-0.0166027073 -0.0240519679
-0.0191219835 -0.0217116689
-0.0216412597 -0.0193713700
-0.0241605359 -0.0170310710
-0.0266798121 -0.0146907720
-0.0291990883 -0.0123504730
-0.0317183645 -0.0100101740
-0.0342376407 -0.0076698750
-0.0342083000 -0.0132806190
-0.0341789592 -0.0188913631
-0.0341496185 -0.0245021071
-0.0341202778 -0.0301128511
-0.0340909371 -0.0357235951
-0.0340615963 -0.0413343391
-0.0340322556 -0.0469450831
-0.0340029149 -0.0525558271
-0.0302287379 -0.0605063092
-0.0264545608 -0.0684567913
-0.0226803838 -0.0764072733
-0.0189062068 -0.0843577554
-0.0151320297 -0.0923082375
-0.0113578527 -0.1002587196
-0.0075836757 -0.1082092017
-0.0038094986 -0.1161596837
-0.0050310065 -0.1205504941
-0.0062525143 -0.1249413045
-0.0074740221 -0.1293321148
-0.0086955299 -0.1337229252
-0.0099170377 -0.1381137355
-0.0111385455 -0.1425045459
-0.0123600533 -0.1468953563
-0.0135815611 -0.1512861666
-0.0177345673 -0.1679878427
-0.0218875735 -0.1846895187
-0.0260405796 -0.2013911947
-0.0301935858 -0.2180928708
-0.0343465920 -0.2347945468
-0.0384995981 -0.2514962229
-0.0426526043 -0.2681978989
-0.0468056105 -0.2848995750
-0.0603819870 -0.2930394010
-0.0739583635 -0.3011792270
-0.0875347400 -0.3093190530
-0.1011111165 -0.3174588790
-0.1146874930 -0.3255987051
-0.1282638695 -0.3337385311
-0.1418402460 -0.3418783571
-0.1554166225 -0.3500181831
-0.1409929824 -0.3598373583
-0.1265693424 -0.3696565335
-0.1121457023 -0.3794757087
-0.0977220623 -0.3892948840
-0.0832984222 -0.3991140592
-0.0688747822 -0.4089332344
-0.0544511421 -0.4187524096
-0.0400275021 -0.4285715848
-0.0558157072 -0.4331352277
-0.0716039123 -0.4376988706
-0.0873921174 -0.4422625135
-0.1031803225 -0.4468261564
-0.1189685276 -0.4513897992
-0.1347567327 -0.4559534421
-0.1505449378 -0.4605170850
-0.1663331429 -0.4650807279
-0.1567041031 -0.4716295393
-0.1470750634 -0.4781783506
-0.1374460236 -0.4847271620
-0.1278169839 -0.4912759734
-0.1181879441 -0.4978247848
-0.1085589043 -0.5043735962
-0.0989298646 -0.5109224076
-0.0893008248 -0.5174712190
-0.0984770317 -0.5222601326
-0.1076532386 -0.5270490462
-0.1168294455 -0.5318379598
-0.1260056524 -0.5366268734
-0.1351818593 -0.5414157871
-0.1443580662 -0.5462047007
-0.1535342730 -0.5509936143
-0.1627104799 -0.5557825279
-0.1752541442 -0.5583581739
-0.1877978085 -0.5609338199
-0.2003414729 -0.5635094659
-0.2128851372 -0.5660851118
-0.2254288015 -0.5686607578
-0.2379724658 -0.5712364038
-0.2505161301 -0.5738120498
-0.2630597944 -0.5763876957
-0.2576101195 -0.5609817268
-0.2521604446 -0.5455757578
-0.2467107697 -0.5301697889
-0.2412610948 -0.5147638200
-0.2358114199 -0.4993578510
-0.2303617450 -0.4839518821
-0.2249120701 -0.4685459131
-0.2194623952 -0.4531399442
-0.2164547806 -0.4465132908
-0.2134471660 -0.4398866375
-0.2104395514 -0.4332599842
-0.2074319367 -0.4266333308
-0.2044243221 -0.4200066775
-0.2014167075 -0.4133800241
-0.1984090929 -0.4067533708
-0.1954014783 -0.4001267174
-0.1959208875 -0.3884120074
-0.1964402967 -0.3766972975
-0.1969597059 -0.3649825875
-0.1974791151 -0.3532678775
-0.1979985243 -0.3415531675
-0.1985179334 -0.3298384575
-0.1990373426 -0.3181237475
-0.1995567518 -0.3064090376
-0.1905043076 -0.2922368430
-0.1814518634 -0.2780646484
-0.1723994192 -0.2638924538
-0.1633469750 -0.2497202592
-0.1542945307 -0.2355480646
-0.1452420865 -0.2213758700
-0.1361896423 -0.2072036754
-0.1271371981 -0.1930314807
-0.1128507565 -0.1843834445
-0.0985643149 -0.1757354083
-0.0842778733 -0.1670873721
-0.0699914317 -0.1584393358
-0.0557049901 -0.1497912996
-0.0414185485 -0.1411432634
-0.0271321068 -0.1324952272
-0.0128456652 -0.1238471909
-0.0109721440 -0.1120948262
-0.0090986228 -0.1003424614
-0.0072251015 -0.0885900966
-0.0053515803 -0.0768377318
-0.0034780590 -0.0650853670
-0.0016045378 -0.0533330023
0.0002689834 -0.0415806375
0.0021425047 -0.0298282727
0.0017400109 -0.0259650366
0.0013375170 -0.0221018004
0.0009350232 -0.0182385643
0.0005325294 -0.0143753282
0.0001300356 -0.0105120921
-0.0002724582 -0.0066488559
-0.0006749520 -0.0027856198
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
0.0022157687 -0.0011790354
0.0055089833 -0.0034356872
0.0088021979 -0.0056923389
0.0120954125 -0.0079489907
0.0153886271 -0.0102056424
0.0186818417 -0.0124622942
0.0219750563 -0.0147189459
0.0252682709 -0.0169755977
0.0384179071 -0.0196000192
0.0515675432 -0.0222244408
0.0647171794 -0.0248488623
0.0778668156 -0.0274732838
0.0910164518 -0.0300977054
0.1041660879 -0.0327221269
0.1173157241 -0.0353465484
0.1304653603 -0.0379709700
0.1279659900 -0.0368285670
0.1254666197 -0.0356861639
0.1229672494 -0.0345437609
0.1204678792 -0.0334013579
0.1179685089 -0.0322589549
0.1154691386 -0.0311165519
0.1129697683 -0.0299741488
0.1104703981 -0.0288317458
0.1278989059 -0.0332803228
0.1453274138 -0.0377288997
0.1627559217 -0.0421774766
0.1801844296 -0.0466260535
0.1976129374 -0.0510746304
0.2150414453 -0.0555232074
0.2324699532 -0.0599717843
0.2498984611 -0.0644203612
0.2514213717 -0.0493742089
0.2529442823 -0.0343280566
0.2544671930 -0.0192819043
0.2559901036 -0.0042357520
0.2575130142 0.0108104003
0.2590359249 0.0258565526
0.2605588355 0.0409027049
0.2620817461 0.0559488572
0.2832734528 0.0449870340
0.3044651596 0.0340252107
0.3256568663 0.0230633875
0.3468485730 0.0121015642
0.3680402798 0.0011397410
0.3892319865 -0.0098220822
0.4104236932 -0.0207839055
0.4316154000 -0.0317457287
0.4318420968 -0.0273595351
0.4320687936 -0.0229733414
0.4322954904 -0.0185871477
0.4325221872 -0.0142009541
0.4327488840 -0.0098147604
0.4329755807 -0.0054285668
0.4332022775 -0.0010423731
0.4334289743 0.0033438206
0.4641158000 -0.0037431539
0.4948026256 -0.0108301283
0.5254894512 -0.0179171028
0.5561762768 -0.0250040772
0.5868631024 -0.0320910517
0.6175499280 -0.0391780261
0.6482367536 -0.0462650006
0.6789235793 -0.0533519750
0.7055635370 -0.0573036793
0.7322034947 -0.0612553836
0.7588434525 -0.0652070879
0.7854834102 -0.0691587921
0.8121233680 -0.0731104964
0.8387633257 -0.0770622007
0.8654032834 -0.0810139050
0.8920432412 -0.0849656093
0.8851420511 -0.0756914412
0.8782408611 -0.0664172730
0.8713396710 -0.0571431049
0.8644384809 -0.0478689367
0.8575372909 -0.0385947686
0.8506361008 -0.0293206004
0.8437349108 -0.0200464323
0.8368337207 -0.0107722641
0.8654465079 0.0007332529
0.8940592952 0.0122387699
0.9226720824 0.0237442870
0.9512848696 0.0352498040
0.9798976569 0.0467553211
1.0085104441 0.0582608381
1.0371232313 0.0697663551
1.0657360185 0.0812718722
1.0905743758 0.0764389114
1.1154127331 0.0716059506
1.1402510904 0.0667729898
1.1650894477 0.0619400290
1.1899278050 0.0571070682
1.2147661623 0.0522741074
1.2396045196 0.0474411466
1.2644428769 0.0426081858
1.2780021579 0.0443858693
1.2915614388 0.0461635529
1.3051207198 0.0479412364
1.3186800008 0.0497189200
1.3322392817 0.0514966035
1.3457985627 0.0532742871
1.3593578437 0.0550519706
1.3729171247 0.0568296541
1.4048829405 0.0504745819
1.4368487564 0.0441195097
1.4688145723 0.0377644374
1.5007803882 0.0314093652
1.5327462041 0.0250542929
1.5647120199 0.0186992207
1.5966778358 0.0123441484
1.6286436517 0.0059890762
1.6125730409 0.0044163534
1.5965024300 0.0028436306
1.5804318192 0.0012709079
1.5643612084 -0.0003018149
1.5482905975 -0.0018745377
1.5322199867 -0.0034472604
1.5161493758 -0.0050199832
1.5000787650 -0.0065927060
1.5153224855 -0.0147418597
1.5305662061 -0.0228910134
1.5458099266 -0.0310401672
1.5610536471 -0.0391893209
1.5762973676 -0.0473384746
1.5915410881 -0.0554876283
1.6067848087 -0.0636367821
1.6220285292 -0.0717859358
1.6000450195 -0.0770714804
1.5780615098 -0.0823570251
1.5560780001 -0.0876425697
1.5340944904 -0.0929281143
1.5121109807 -0.0982136590
1.4901274710 -0.1034992036
1.4681439613 -0.1087847483
1.4461604516 -0.1140702929
1.4182550007 -0.1081717101
1.3903495499 -0.1022731273
1.3624440991 -0.0963745445
1.3345386482 -0.0904759617
1.3066331974 -0.0845773789
1.2787277466 -0.0786787962
1.2508222957 -0.0727802134
1.2229168449 -0.0668816306
1.1973981279 -0.0658334995
1.1718794109 -0.0647853683
1.1463606939 -0.0637372372
1.1208419768 -0.0626891061
1.0953232598 -0.0616409750
1.0698045428 -0.0605928439
1.0442858258 -0.0595447128
1.0187671088 -0.0584965816
1.0150431707 -0.0519728748
1.0113192326 -0.0454491679
1.0075952946 -0.0389254611
1.0038713565 -0.0324017542
1.0001474184 -0.0258780474
0.9964234803 -0.0193543405
0.9926995423 -0.0128306337
0.9889756042 -0.0063069268
0.9813383262 -0.0146830331
0.9737010481 -0.0230591393
0.9660637701 -0.0314352455
0.9584264921 -0.0398113517
0.9507892140 -0.0481874580
0.9431519360 -0.0565635642
0.9355146580 -0.0649396704
0.9278773800 -0.0733157766
0.8929513794 -0.0680299642
0.8580253789 -0.0627441517
0.8230993783 -0.0574583392
0.7881733778 -0.0521725267
0.7532473772 -0.0468867143
0.7183213767 -0.0416009018
0.6833953761 -0.0363150893
0.6484693756 -0.0310292768
0.6201181341 -0.0370998198
0.5917668926 -0.0431703628
0.5634156511 -0.0492409058
0.5350644096 -0.0553114488
0.5067131680 -0.0613819918
0.4783619265 -0.0674525348
0.4500106850 -0.0735230778
0.4216594435 -0.0795936208
0.4049838244 -0.0773081589
0.3883082053 -0.0750226971
0.3716325862 -0.0727372353
0.3549569671 -0.0704517735
0.3382813481 -0.0681663116
0.3216057290 -0.0658808498
0.3049301099 -0.0635953880
0.2882544908 -0.0613099262
0.2685308495 -0.0583925566
0.2488072082 -0.0554751871
0.2290835668 -0.0525578176
0.2093599255 -0.0496404481
0.1896362842 -0.0467230785
0.1699126429 -0.0438057090
0.1501890016 -0.0408883395
0.1304653603 -0.0379709700
0.1387213468 -0.0397142266
0.1469773334 -0.0414574833
0.1552333199 -0.0432007399
0.1634893065 -0.0449439966
0.1717452930 -0.0466872532
0.1800012796 -0.0484305099
0.1882572661 -0.0501737666
0.1965132527 -0.0519170232
0.1863968192 -0.0428898246
0.1762803857 -0.0338626260
0.1661639523 -0.0248354274
0.1560475188 -0.0158082288
0.1459310854 -0.0067810302
0.1358146519 0.0022461684
0.1256982185 0.0112733671
0.1155817850 0.0203005657
0.1071002855 0.0211077134
0.0986187859 0.0219148610
0.0901372864 0.0227220087
0.0816557869 0.0235291564
0.0731742873 0.0243363041
0.0646927878 0.0251434518
0.0562112883 0.0259505995
0.0477297888 0.0267577472
0.0410008791 0.0264748579
0.0342719694 0.0261919686
0.0275430598 0.0259090793
0.0208141501 0.0256261900
0.0140852405 0.0253433008
0.0073563308 0.0250604115
0.0006274212 0.0247775222
-0.0061014885 0.0244946329
-0.0067700178 0.0231465531
-0.0074385470 0.0217984734
-0.0081070763 0.0204503936
-0.0087756056 0.0191023138
-0.0094441349 0.0177542341
-0.0101126641 0.0164061543
-0.0107811934 0.0150580745
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0114497227 0.0137099947
-0.0147155601 0.0135749463
-0.0179813974 0.0134398978
-0.0212472348 0.0133048494
-0.0245130721 0.0131698009
-0.0277789095 0.0130347525
-0.0310447469 0.0128997040
-0.0343105842 0.0127646556
-0.0375764216 0.0126296071
-0.0330140496 0.0111856082
-0.0284516776 0.0097416094
-0.0238893057 0.0082976106
-0.0193269337 0.0068536117
-0.0147645617 0.0054096129
-0.0102021898 0.0039656140
-0.0056398178 0.0025216152
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0023739805 0.0026566636
-0.0036705151 0.0042357109
-0.0049670497 0.0058147582
-0.0062635843 0.0073938055
-0.0075601189 0.0089728528
-0.0088566535 0.0105519001
-0.0101531881 0.0121309474
-0.0114497227 0.0137099947
-0.0147155601 0.0135749463
-0.0179813974 0.0134398978
-0.0212472348 0.0133048494
-0.0245130721 0.0131698009
-0.0277789095 0.0130347525
-0.0310447469 0.0128997040
-0.0343105842 0.0127646556
-0.0375764216 0.0126296071
-0.0504870697 0.0239473066
-0.0633977178 0.0352650061
-0.0763083659 0.0465827056
-0.0892190140 0.0579004051
-0.1021296621 0.0692181047
-0.1150403102 0.0805358042
-0.1279509583 0.0918535037
-0.1408616064 0.1031712032
-0.1411613720 0.0995534737
-0.1414611376 0.0959357442
-0.1417609032 0.0923180146
-0.1420606688 0.0887002851
-0.1423604345 0.0850825556
-0.1426602001 0.0814648261
-0.1429599657 0.0778470965
-0.1432597313 0.0742293670
-0.1459059324 0.0731528645
-0.1485521335 0.0720763619
-0.1511983346 0.0709998594
-0.1538445357 0.0699233568
-0.1564907368 0.0688468543
-0.1591369379 0.0677703518
-0.1617831390 0.0666938492
-0.1644293401 0.0656173467
-0.1565325617 0.0638344163
-0.1486357833 0.0620514859
-0.1407390049 0.0602685554
-0.1328422265 0.0584856250
-0.1249454480 0.0567026946
-0.1170486696 0.0549197642
-0.1091518912 0.0531368338
-0.1012551128 0.0513539034
-0.0982142387 0.0453362827
-0.0951733646 0.0393186621
-0.0921324906 0.0333010414
-0.0890916165 0.0272834208
-0.0860507424 0.0212658001
-0.0830098684 0.0152481795
-0.0799689943 0.0092305588
-0.0769281202 0.0032129382
-0.0704866949 0.0037299722
-0.0640452695 0.0042470063
-0.0576038441 0.0047640403
-0.0511624187 0.0052810744
-0.0447209934 0.0057981085
-0.0382795680 0.0063151425
-0.0318381426 0.0068321766
-0.0253967172 0.0073492106
-0.0223568083 0.0065652614
-0.0193168994 0.0057813121
-0.0162769905 0.0049973628
-0.0132370815 0.0042134135
-0.0101971726 0.0034294642
-0.0071572637 0.0026455149
-0.0041173548 0.0018615656
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0010774458 0.0010776163
-0.0056398178 0.0025216152
-0.0102021898 0.0039656140
-0.0147645617 0.0054096129
-0.0193269337 0.0068536117
-0.0238893057 0.0082976106
-0.0284516776 0.0097416094
-0.0330140496 0.0111856082
-0.0375764216 0.0126296071
-0.0422887386 0.0191428368
-0.0470010556 0.0256560665
-0.0517133726 0.0321692961
-0.0564256897 0.0386825258
-0.0611380067 0.0451957555
-0.0658503237 0.0517089852
-0.0705626407 0.0582222148
-0.0752749577 0.0647354445
-0.0927804970 0.0773528659
-0.1102860364 0.0899702874
-0.1277915757 0.1025877088
-0.1452971150 0.1152051302
-0.1628026543 0.1278225516
-0.1803081936 0.1404399730
-0.1978137329 0.1530573944
-0.2153192722 0.1656748158
-0.2252334789 0.1702264279
-0.2351476855 0.1747780399
-0.2450618921 0.1793296519
-0.2549760987 0.1838812639
-0.2648903054 0.1884328759
-0.2748045120 0.1929844880
-0.2847187186 0.1975361000
-0.2946329252 0.2020877120
-0.3083703891 0.2198840102
-0.3221078530 0.2376803084
-0.3358453169 0.2554766065
-0.3495827808 0.2732729047
-0.3633202448 0.2910692029
-0.3770577087 0.3088655011
-0.3907951726 0.3266617993
-0.4045326365 0.3444580974
-0.4381292123 0.3723481920
-0.4717257881 0.4002382866
-0.5053223639 0.4281283811
-0.5389189397 0.4560184757
-0.5725155156 0.4839085703
-0.6061120914 0.5117986648
-0.6397086672 0.5396887594
-0.6733052430 0.5675788540
-0.7028557678 0.5708074504
-0.7324062925 0.5740360468
-0.7619568173 0.5772646432
-0.7915073420 0.5804932396
-0.8210578668 0.5837218360
-0.8506083915 0.5869504324
-0.8801589162 0.5901790288
-0.9097094410 0.5934076252
-0.9217879894 0.5955760940
-0.9338665379 0.5977445628
-0.9459450863 0.5999130317
-0.9580236348 0.6020815005
-0.9701021832 0.6042499693
-0.9821807316 0.6064184381
-0.9942592801 0.6085869069
-1.0063378285 0.6107553758
-0.9807453429 0.6020550118
-0.9551528572 0.5933546479
-0.9295603716 0.5846542840
-0.9039678860 0.5759539201
-0.8783754003 0.5672535561
-0.8527829147 0.5585531922
-0.8271904291 0.5498528283
-0.8015979434 0.5411524644
-0.7863563598 0.5261469331
-0.7711147763 0.5111414019
-0.7558731927 0.4961358707
-0.7406316091 0.4811303394
-0.7253900255 0.4661248082
-0.7101484419 0.4511192770
-0.6949068583 0.4361137457
-0.6796652748 0.4211082145
-0.6677607413 0.4116763860
-0.6558562079 0.4022445576
-0.6439516745 0.3928127291
-0.6320471411 0.3833809007
-0.6201426076 0.3739490722
-0.6082380742 0.3645172438
-0.5963335408 0.3550854153
-0.5844290074 0.3456535869
-0.5942770262 0.3385888830
-0.6041250450 0.3315241792
-0.6139730639 0.3244594753
-0.6238210827 0.3173947715
-0.6336691016 0.3103300676
-0.6435171204 0.3032653638
-0.6533651393 0.2962006600
-0.6632131581 0.2891359561
-0.6253335824 0.2678461368
-0.5874540067 0.2465563174
-0.5495744310 0.2252664981
-0.5116948553 0.2039766787
-0.4738152796 0.1826868594
-0.4359357039 0.1613970401
-0.3980561282 0.1401072207
-0.3601765525 0.1188174014
-0.3630228302 0.1209762369
-0.3658691080 0.1231350725
-0.3687153857 0.1252939081
-0.3715616635 0.1274527436
-0.3744079412 0.1296115792
-0.3772542190 0.1317704148
-0.3801004967 0.1339292503
-0.3829467744 0.1360880859
-0.3865051923 0.1362714471
-0.3900636101 0.1364548083
-0.3936220280 0.1366381695
-0.3971804458 0.1368215307
-0.4007388637 0.1370048920
-0.4042972815 0.1371882532
-0.4078556994 0.1373716144
-0.4114141172 0.1375549756
-0.3961902738 0.1296709198
-0.3809664303 0.1217868640
-0.3657425869 0.1139028082
-0.3505187435 0.1060187525
-0.3352949000 0.0981346967
-0.3200710566 0.0902506409
-0.3048472132 0.0823665851
-0.2896233697 0.0744825293
-0.2662001190 0.0690569119
-0.2427768683 0.0636312946
-0.2193536176 0.0582056772
-0.1959303669 0.0527800598
-0.1725071162 0.0473544425
-0.1490838654 0.0419288251
-0.1256606147 0.0365032077
-0.1022373640 0.0310775904

